UMEDA: Unified Multi-modal Efficient Data Fusion for Privacy-Preserving Graph Federated Learning via Spectral-Gated Attention and Diffusion-Based Operator Alignment

Device-free localization trains models from heterogeneous wireless and visual sensors (e.g., Wi-Fi, LiDAR) distributed across edge devices. Federated learning offers a privacy-respecting framework, but is brittle when clients differ in sensor modality and resolution, when their data distributions drift, and when privacy noise destroys the structural signal needed for localization. We propose UMEDA, a graph federated learning framework in which clients form nodes of a global graph that share a continuous integral operator, and aggregation is reformulated as spectral signal processing on this operator. Each client encodes its local sensors with a linear-attention layer whose kernel spectrum is low-rank filtered, suppressing modality-specific residuals so clients with different sensors align in a common low-rank subspace. The server then aggregates client updates via a diffusion model over the kernel's spectral coefficients, treating updates as discretizations of a shared operator rather than topology-bound weights -- this absorbs varying graph sizes and missing modalities without node-wise correspondence. To balance privacy and utility, we add an anisotropic differential-privacy mechanism that projects noise preferentially into the null space of the signal subspace, preserving dominant eigendirections while ensuring formal $(\epsilon, \delta)$-DP under gradient clipping. On MM-Fi and the RELI11D out-of-distribution benchmark, UMEDA outperforms state-of-the-art federated baselines in accuracy, convergence, and communication efficiency, particularly under high modality heterogeneity and tight privacy budgets.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1--2 sentence) justification right after your answer (even for \answerNA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will also be asked to include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While \answerYes{} is generally preferable to \answerNo{}, it is perfectly acceptable to answer \answerNo{} provided a proper justification is given (e.g., error bars are not reported because it would be too computationally expensive'' or ``we were unable to find the license for the dataset we used''). In general, answering \answerNo{} or \answerNA{} is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and Section~\ref{sec:method} introduce the three components (SGLT, Diff-GNO, SP-DP) and the corresponding empirical claims (accuracy, convergence, privacy--utility frontier, communication efficiency). All claims are substantiated by Tables~\ref{tab:main}--\ref{tab:comm} and Figure~\ref{fig:robustness_analyses}; assumptions and scope are stated in Sec.~\ref{sec:method} and Appendix~\ref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitations are discussed in Appendix~\ref{sec:limitations}, covering compute and systems overhead, block-specific aggregation assumptions, sensitivity to diffusion hyperparameters, DP composition over rounds, and operator mismatch under extreme modality shifts.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Theorems~\ref{thm:eym}, \ref{thm:spdp_dp}, Corollary~\ref{cor:hard_gate}, and Lemmas~\ref{lem:soft_gate_bound}, \ref{lem:size_free} are stated with explicit assumptions in Section~\ref{sec:method} and proven in Appendix~\ref{app:proofs} (\ref{app:sglt_proof}, \ref{app:dp_proof}, \ref{app:res_indep}). The SP-DP proof relies explicitly on the data-independence of the projection basis $\mathbf{P}_{\mathcal{S}}$, which is stated as a hypothesis.   
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sec.~\ref{sec:setup} specifies the federated simulation ($K=100$ clients, sampling rate $q=0.4$, $T=1000$ rounds, $E=100$ local steps), model architecture (SGLT $d=256$, 8 heads, FAVOR+ $m=256$), VE-SDE schedule (Eq.~\eqref{eq:ve_sigma_closed}), DP calibration (Eq.~\eqref{eq:dp_calib}), and full hyperparameters $(\tau_s,\beta,C,\kappa)$. Datasets MM-Fi and RELI11D are publicly available. All algorithms are stated in Alg.~\ref{alg:umeda}--\ref{alg:spdp}.   
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Anonymized code is not released at submission time to preserve double-blind review. We will release the codebase, configuration files, and reproduction scripts upon acceptance. Both datasets (MM-Fi~\cite{YangNeurIPS23} and RELI11D~\cite{YenCVPR24}) are publicly available from their authors. The paper provides full hyperparameters and pseudocode (Alg.~\ref{alg:umeda}, \ref{alg:spdp}) sufficient for re-implementation.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sec.~\ref{sec:setup} gives data splits (Dirichlet $\alpha$, three client types A/B/C), optimizer (AdamW, lr $10^{-3}$, weight decay $10^{-4}$, batch size $64$), training horizon, server step size, DP budgets, and architectural choices. Hyperparameter ablations and sensitivity analyses are in Appendix~\ref{app:exp}.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All main results (Tables~\ref{tab:main}, \ref{tab:reli11d}, Figure~\ref{fig:robustness_analyses}) report mean$\pm$1 standard deviation over 3 random seeds, computed from independent training runs with different initialization and client sampling. Standard deviation (not standard error) is reported, as stated in figure and table captions.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Per-round server wall-clock and per-client latency/peak memory are reported in Appendix~\ref{app:scalability} (Table~\ref{tab:a_scalability}) and Appendix~A.10 (Table~\ref{tab:a_cost}). Experiments were run on a single NVIDIA RTX 4500 Ada workstation with 24GB VRAM; full $T=1000$ round runs take approximately 18 GPU-hours per seed at $K=100$ clients. Total compute including ablations and failed exploratory runs is approximately 800 GPU-hours.     
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conforms to the NeurIPS Code of Ethics. We use only publicly released datasets (MM-Fi, RELI11D) collected with their authors' IRB approval; no new human-subject data is collected. Privacy implications of device-free sensing are explicitly addressed in Appendix~\ref{app:societal_impact}.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Both positive impacts (ambient health monitoring, accessibility, infrastructure-light navigation) and potential risks (non-consensual surveillance via passive Wi-Fi sensing, fairness across demographics) are discussed in Appendix~\ref{app:societal_impact}, along with mitigation strategies (formal DP guarantees, secure aggregation, deployment governance).    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release pre-trained models, scraped datasets, or generative content. The released artifact (upon acceptance) is a federated training algorithm whose primary effect is to \emph{strengthen} privacy in existing sensing pipelines; misuse risk is below the threshold for safeguarded release.   
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All datasets and baseline implementations are cited with their original publications: MM-Fi~\cite{YangNeurIPS23} (CC BY-NC 4.0), RELI11D~\cite{YenCVPR24} (research use), MetaFi++~\cite{Wang2022MetaFiPlusPlus}, X-Fi~\cite{xfi2024}, and federated baselines (FedAvg, FedProx, etc.). We use these assets within their stated terms of use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper introduces algorithms and methodology; no new datasets, pre-trained models, or other assets are released at submission time. Code release upon acceptance will follow standard documentation practices (README, configs, environment specification).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or new human-subjects research. We use only previously published datasets that already include their own consent and IRB documentation.    
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new human-subjects data collection is performed. The datasets used (MM-Fi, RELI11D) carry IRB approval from their original creators.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  LLMs were used only as writing aids (grammar editing, LaTeX formatting) and not as any component of the core methodology, model architecture, or experimental analysis.   
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> paper_content/00_abstract.tex <==


\begin{abstract}
    Device-free localization (DFL) requires learning robust representations from heterogeneous sensor modalities (e.g., Wi-Fi, LiDAR) under strict privacy constraints. Existing federated approaches often fail to generalize due to \textbf{discretization heterogeneity} (varying sensor modalities and resolutions) , \textbf{non-IID distribution shifts}, and the \textbf{privacy-utility trade-off}. We propose UMEDA, a privacy-preserving graph federated learning (GFL) framework that reformulates data fusion by integrating spectral signal processing into graph foundation models. First, to reconcile multi-modal heterogeneity, we devise a \textbf{Spectral-Gated Linear Transformer (SGLT)}. Instead of standard attention, SGLT incorporates a low-rank filtering mechanism on the kernel's singular spectrum. By explicitly attenuating modality-specific residual subspaces via this spectral gating, SGLT introduces a strong inductive bias for learning shared local semantic structures alignment across clients. Second, to mitigate non-IID drift, we propose a \textbf{Diffusion-based Graph Neural Operator (Diff-GNO)} for global aggregation. Unlike standard diffusion models, which are limited to fixed dimensions, Diff-GNO learns a resolution-independent generative mapping in the function space, parameterized by a shared operator backbone. This enables the global model to generate intermediate latent representations that reduce client distribution shift across resolutions and modalities, effectively handling varying graph sizes and missing modalities without requiring node-wise correspondence. Third, we balance the privacy-utility trade-off via \textbf{Subspace-Projected Differential Privacy (SP-DP)}. Leveraging the spectral decomposition from SGLT, we design an anisotropic mechanism that projects noise preferentially into directions with lower utility impact. This approach preserves the dominant eigenspaces critical for localization accuracy while ensuring formal $(\epsilon, \delta)$-differential privacy guarantees under bounded update sensitivity via gradient clipping. Empirical evaluations on MM-Fi and RELI11D benchmarks demonstrate that UMEDA significantly outperforms state-of-the-art federated baselines in accuracy and convergence, particularly in scenarios with high modal heterogeneity and strict privacy budgets, successfully reconciling the trade-off between privacy guarantees, communication efficiency, and cross-modal generalization.
\end{abstract}




==> paper_content/01_introduction.tex <==
\section{Introduction}


Device-free localization (DFL) infers a person's position, pose, and activity from ambient sensor streams—Wi-Fi channel state information~\citep{JiangMobiCom20,Wang2022MetaFiPlusPlus,MFFALoc,LocFree}, millimeter-wave radar~\citep{ChenMM22,LeeWACV23}, and LiDAR or depth point clouds~\citep{Wang2018,YenCVPR24}—without requiring users to wear any device. Fusing these modalities is attractive because each sensor compensates for the others' blind spots~\citep{YangNeurIPS23,AnNeurIPS22,chen2023immfusion}, but it raises a problem that is fundamentally not centralized: the raw streams reveal where a person is, what they are doing, and what their environment looks like, and they are too bandwidth-heavy to ship to a central server. Federated learning (FL)~\citep{McMahan2017FedAvg} is the natural framework, but standard FL does not match three properties of multi-modal sensing.

\textbf{Clients have different sensors and different resolutions.} A Wi-Fi client and a LiDAR client do not produce comparable feature tensors, and even within one modality the spatial resolution varies across devices. Generic FL methods such as FedAvg~\citep{McMahan2017FedAvg}, FedProx~\citep{Li2020FedProx}, and SCAFFOLD~\citep{Karimireddy2020SCAFFOLD} aggregate by averaging weights and assume every client trains the same architecture on the same input shape. Graph federated learning (GFL)~\citep{Chen2023FedGraphSurvey,Li2024FederatedGNNs}—where clients are treated as nodes of a global graph and aggregation is structure-aware~\citep{FedGTA,FedTAD,Qiu2022FedGraphNN}—relaxes the homogeneity assumption, but existing GFL methods build the inter-client graph from heuristic similarity scores that become unstable when client A produces Wi-Fi spectrograms and client B produces sparse LiDAR point clouds. There is no representation in which the two clients' updates can be directly compared.

\textbf{Client distributions drift.} Different rooms, body sizes, and sensor placements shift the joint distribution of inputs and labels. Optimizer-based fixes~\citep{Li2020FedProx,Karimireddy2020SCAFFOLD,Reddi2021FedOpt,Acar2021FedDyn,Li2021MOON} constrain weight-space updates but do not align the underlying representations. Recent generative FL approaches~\citep{weng2024feddiff,pinaya2024feddm,chen2025fedbip} use diffusion models to synthesize alignment data on the server, but operate in fixed-dimensional Euclidean space and do not transfer to graphs of varying size. Neural operators~\citep{kovachki2021neuraloperator,li2020mgno} provide a resolution-independent function-space alternative, yet have been used for supervised PDE regression rather than for federated distribution alignment.

\textbf{Differential privacy is misaligned with the threat model.} In DFL, the server is allowed to know that a client is participating, but should not be able to reconstruct what that client looks like, what action the person performs, or where they are in the room. Standard DP mechanisms~\citep{Geyer2017,Dwork2014DP,Abadi2016MomentsAccountant,andrew2022adaptiveclipping} clip updates and inject isotropic Gaussian noise; this protects all directions equally, including the low-rank directions that carry the localization signal. The result is that strong privacy budgets erase the very structure needed for accurate pose and position estimation.

\textbf{Our approach.} We propose \textbf{UMEDA}, a graph federated learning framework where clients are nodes of a global graph that share a continuous integral operator (rather than a fixed weight tensor), and aggregation is reformulated as spectral signal processing on that operator. The hypothesis is that while sensors discretize the world differently, the physical kernel relating environment to observation is shared, so federation should happen in operator space, not weight space. Concretely, UMEDA contributes:

\begin{itemize}
    \item A linear-attention encoder whose kernel spectrum is low-rank filtered (\textbf{SGLT}). The filter suppresses modality-specific high-frequency components, embedding clients with different sensors in a common low-rank subspace.
    \item A diffusion model over the kernel's spectral coefficients (\textbf{Diff-GNO}). Treating client updates as discretizations of a shared operator, the server aggregates by generative denoising, handling varying graph sizes and missing modalities without node-wise correspondence.
    \item An anisotropic DP mechanism (\textbf{SP-DP}). Noise is projected into the null space of the public signal subspace, hiding client-specific scene appearance, motion, and position while preserving the eigendirections that carry localization utility, under formal $(\epsilon,\delta)$-DP.
\end{itemize}

On MM-Fi~\citep{YangNeurIPS23} and the RELI11D out-of-distribution benchmark~\citep{YenCVPR24}, UMEDA outperforms state-of-the-art federated, graph-FL, and DP-FL baselines in accuracy, convergence, and communication, particularly under high modality heterogeneity and tight privacy budgets. Figure~\ref{fig:arch_overview} shows the end-to-end pipeline; Figure~\ref{fig:modules} summarizes the three components.

==> paper_content/02_related_work.tex <==
\section{Related Work}



==> paper_content/02_related_work_short.tex <==
\section{Related Work}


\subsection{Graph Representation Learning for Heterogeneous Signals}
Learning unified representations from multi-modal sensor data (e.g., LiDAR point clouds, Wi-Fi CSI, mmWave) is fundamentally a problem of reconciling \textbf{discretization heterogeneity}. Early approaches relied on grid-based voxelization or multi-view projections, which discard fine-grained topological information. Point-based methods, such as Point-GNN \cite{Shi2020PointGNN} and Graph Attention Convolution \cite{GraphAttentionConvolution}, construct nearest-neighbor graphs to capture local geometry via message passing. However, these methods typically assume homogeneous node features and struggle to align modalities with vastly different densities and noise profiles.

While Transformers have been adapted for graphs to model long-range dependencies \cite{Wang2022GTNet, 2023SuperpointTransformer}, standard self-attention scales quadratically and is sensitive to high-frequency sensor noise. Recent linear attention mechanisms (e.g., Performer, Nyströmformer) reduce complexity but lack inductive biases for \textbf{spectral filtering}. They treat all spectral components equally, failing to distinguish between the shared low-rank semantic subspace (the underlying human pose) and modality-specific high-frequency artifacts (sensor noise). This limitation necessitates a spectral-gated approach that can explicitly filter residual subspaces to ensure robust cross-modal alignment.

\subsection{Federated Learning under Non-IID Concept Drift}
Federated Learning (FL) faces significant challenges when client data is non-IID (independent and identically distributed). Optimization-based methods like FedProx \cite{Li2020} and Scaffold \cite{Karimireddy2020} attempt to constrain local updates, but they operate in the weight space and struggle with severe concept drift caused by environmental variations in sensing data. Recently, \textbf{Generative Federated Learning }has emerged as a promising direction, where diffusion models or GANs are used to synthesize data or features to augment the server-side distribution. However, standard diffusion models operate on fixed-dimensional Euclidean spaces (e.g., images of resolution ), making them ill-suited for graph data where the number of nodes and topology vary across clients. \textbf{Neural Operators}, such as the Graph Neural Operator (GNO), offer a resolution-independent alternative by learning mappings between infinite-dimensional function spaces. While GNOs have been applied to partial differential equations (PDEs), their potential for \textbf{generative distribution alignment} in FL remains underexplored. Existing works utilize GNOs primarily for supervised regression, missing the opportunity to leverage operator-theoretic foundations to bridge the distribution gap between clients with heterogeneous discretizations.

\subsection{Privacy-Utility Trade-offs in Geometric Deep Learning}
Deploying graph learning in privacy-sensitive environments requires rigorous guarantees, typically formalized via Differential Privacy (DP). Standard approaches, such as DP-SGD, enforce privacy by clipping gradients and injecting isotropic Gaussian noise \cite{Geyer2017}. In the context of geometric deep learning, however, isotropic noise is detrimental because it perturbs all spectral components equally. Since the structural utility of a graph (e.g., localization geometry) is often concentrated in the \textbf{dominant eigenspace}, uniform perturbation yields a poor privacy-utility trade-off.

Recent topology-aware privacy mechanisms attempt to preserve graph structure by adjusting noise based on edge existence or node degrees \cite{Chen2023FedGraphSurvey}. Yet, these methods largely focus on structural anonymity (hiding links) rather than the \textbf{semantic utility} of node features in a foundation model context. There remains a lack of mechanisms that leverage \textbf{subspace projections} to confine noise to the null space of the signal, thereby masking sensitive updates without destroying the low-rank geometric information essential for downstream tasks like localization and pose estimation.


\subsection{Graph Federated Learning via Topology-Aware Aggregation}
While standard Federated Learning treats clients as independent, isolated entities during aggregation (e.g., FedAvg), **Graph Federated Learning (GFL)** explicitly models the underlying correlations between clients as a global graph, where nodes represent clients and edges encode statistical or physical dependencies. Comprehensive surveys have categorized these approaches, highlighting the shift from parameter averaging to structure-aware fusion \cite{Chen2023FedGraphSurvey, Li2024FederatedGNNs}.

Recent frameworks have attempted to learn this inter-client topology to guide personalization. For instance, FedGTA and FedTAD propose topology-aware aggregation strategies, leveraging the learned graph structure to re-weight client contributions and mitigate the impact of non-IID data \cite{FedGTA, FedTAD}. To standardize evaluation in this domain, benchmarks such as FedGraphNN \cite{Qiu2022FedGraphNN} and OpenFGL \cite{Zhang2023OpenFGL} provide modular environments for simulating graph-based FL under various data splits.

However, existing GFL methods typically rely on heuristic similarity metrics to construct the client graph, which becomes unstable under **multi-modal heterogeneity** (e.g., when Client A uses Wi-Fi and Client B uses LiDAR). They lack a rigorous mechanism to align clients in a continuous function space. In contrast, UMEDA moves beyond heuristic graph construction by employing a **Diffusion-based Graph Neural Operator** to learn a generative mapping of client relationships, enabling robust topology-aware aggregation even when clients possess disjoint sensor modalities and varying resolutions.

==> paper_content/03_methodology.tex <==
\section{Method}
\label{sec:method}

We formulate the multi-modal Device-Free Localization (DFL) problem within a federated graph learning framework. Let  $\mathcal{C} = \{1, \dots, N\}$ be the set of clients. Each client $k \in \mathcal{C}$ observes a local dataset $\mathcal{D}_k = \{(\mathbf{X}_k^{(i)}, \mathbf{Y}_k^{(i)})\}_{i=1}^{n_k}$, where $\mathbf{X}_k^{(i)}$ represents heterogeneous sensor inputs (e.g., Wi-Fi CSI, LiDAR point clouds) and $\mathbf{Y}_k^{(i)}$ represents the target labels (e.g., 3D coordinates, action classes).

A fundamental challenge is \textbf{discretization heterogeneity}:  $\mathbf{X}_k$ resides in different topological spaces across clients (e.g., $\mathbb{R}^{N_{pts} \times 3}$ for LiDAR vs. $\mathbb{R}^{N_{sub} \times T}$ for Wi-Fi). We propose \textbf{UMEDA}, a framework that maps these heterogeneous inputs into a unified continuous operator space. The overall training objective is to learn a global operator  $\mathcal{G}^*$ that minimizes the expected risk over the client population distribution $\mathcal{P}$:
\begin{equation}
\mathcal{G}^* = \mathop{\arg\min}*{\mathcal{G} \in \mathfrak{F}} \mathbb{E}*{k \sim \mathcal{P}} \left[ \mathcal{L}_k(\mathcal{G}; \mathcal{D}_k) \right],
\end{equation}
where $\mathfrak{F}$ is the hypothesis space of graph operators. UMEDA achieves this via three coupled components: (1) Spectral-Gated Linear Transformer (SGLT) for local alignment, (2) Diffusion-based Graph Neural Operator (Diff-GNO) for global aggregation, and (3) Subspace-Projected Differential Privacy (SP-DP).

\subsection{Spectral-Gated Linear Transformer (SGLT)}
\label{sec:sglt}

To reconcile multi-modal heterogeneity, we define a local encoder $\Phi_k$ that maps discrete inputs $\mathbf{X}_k$ to a latent sequence $\mathbf{H}_k \in \mathbb{R}^{L \times d}$. Standard self-attention suffers from quadratic complexity and overfits to high-frequency sensor noise. We propose \textbf{SGLT}, which incorporates a low-rank spectral filtering mechanism.

\textbf{Linearized Attention via Kernel Approximation.}
Let $\mathbf{Q}, \mathbf{K}, \mathbf{V} \in \mathbb{R}^{L \times d}$ be the query, key, and value matrices. We utilize a linearized attention mechanism via a feature map :
\begin{equation}
\text{SGLT}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \phi(\mathbf{Q}) \left( \phi(\mathbf{K})^\top \mathbf{V} \right).
\end{equation}
The term $\mathbf{M} = \phi(\mathbf{K})^\top \mathbf{V} \in \mathbb{R}^{d \times d}$ encapsulates the global semantic structure. In multi-modal settings, modality-specific noise (e.g., Wi-Fi multipath, LiDAR outliers) manifests as high-frequency perturbations in $\mathbf{M}$.

\textbf{Spectral Gating Mechanism.}
We explicitly attenuate these noise components by performing a singular value decomposition (SVD) on the aggregated semantic matrix $\mathbf{M}$:
\begin{equation}
\mathbf{M} = \mathbf{U} \mathbf{\Sigma} \mathbf{W}^\top, \quad \text{where } \mathbf{\Sigma} = \text{diag}(\sigma_1, \dots, \sigma_d).
\end{equation}
We define a spectral gate $g(\sigma_i) = \mathbb{I}(\sigma_i > \tau)$  that retains only the dominant singular values corresponding to the shared semantic subspace (e.g., human skeletal structure). The filtered matrix $\hat{\mathbf{M}}$ is reconstructed as:
\begin{equation}
\hat{\mathbf{M}} = \mathbf{U} (g(\mathbf{\Sigma}) \odot \mathbf{\Sigma}) \mathbf{W}^\top.
\end{equation}
The final output is  $\mathbf{H}' = \phi(\mathbf{Q})\hat{\mathbf{M}}$. This acts as a strong inductive bias, enforcing the model to learn low-rank structures that are invariant across sensor modalities.

\subsection{Diffusion-based Graph Neural Operator (Diff-GNO)}
\label{sec:diff_gno}

Standard federated aggregation (e.g., FedAvg) fails under \textbf{non-IID concept drift}, where the underlying distribution $P(\mathbf{X}, \mathbf{Y})$ shifts across clients. We model the global aggregation not as parameter averaging, but as a generative process in the function space.

\textbf{Operator-Theoretic Formulation.}
Let $u_k: D \to \mathbb{R}^d$ be the function representing the local model of client  $k$. We aim to find a global transport map $\mathcal{T}$ that aligns local measures  $\mu_k$ to a global barycenter $\mu^*$. We parameterize this via a \textbf{Graph Neural Operator (GNO)} backbone, which learns the integral kernel:
\begin{equation}
(\mathcal{K}u)(x) = \int_D \kappa(x, y) u(y) dy,
\end{equation}
where  is a resolution-independent kernel parameterized by spectral weights.

\textbf{Generative Diffusion Process.}
To bridge the distribution gaps, we treat the aggregation as a reverse-time diffusion process. The global model is updated by sampling from the score-based generative model defined over the operator space:
\begin{equation}
d\mathbf{\Theta}*t = -\nabla*{\mathbf{\Theta}} \mathcal{L}_{\text{score}}(\mathbf{\Theta}) dt + \sqrt{2} d\mathbf{W}_t.
\end{equation}
Here, $\mathbf{\Theta}$ represents the spectral parameters of the GNO. The diffusion process generates "bridge" representations—intermediate latent functions that interpolate between divergent client distributions. This allows UMEDA to synthesize missing modalities and align features across clients with varying graph sizes without requiring node-wise correspondence.

\subsection{Subspace-Projected Differential Privacy (SP-DP)}
\label{sec:sp_dp}

To address the \textbf{privacy-utility trade-off}, we introduce SP-DP. Standard DP mechanisms inject isotropic noise $\eta \sim \mathcal{N}(0, \sigma^2 \mathbf{I})$, which degrades the utility of the dominant semantic features.

\textbf{Anisotropic Noise Injection.}
Leveraging the spectral basis $\mathbf{U}$ derived from SGLT (Sec.~\ref{sec:sglt}), we decompose the gradient update  $\Delta \mathbf{\Theta}$  into a signal subspace $\mathcal{S} = \text{span}(\mathbf{U}_{1:r})$ and a residual (null) subspace  $\mathcal{S}^\perp$. We construct a projected noise covariance matrix $\mathbf{\Sigma}_{\eta}$:
\begin{equation}
\mathbf{\Sigma}*{\eta} = \sigma*{\text{signal}}^2 \mathbf{P}*{\mathcal{S}} + \sigma*{\text{null}}^2 \mathbf{P}*{\mathcal{S}^\perp},
\end{equation}
where $\mathbf{P}*{\mathcal{S}} = \mathbf{U}*{1:r}\mathbf{U}*{1:r}^\top$ is the projection operator. We set $\sigma_{\text{signal}} \ll \sigma_{\text{null}}$.

\textbf{Privacy Guarantee.}
The perturbed update is $\Delta \tilde{\mathbf{\Theta}} = \text{Clip}(\Delta \mathbf{\Theta}) + \mathcal{N}(0, \mathbf{\Sigma}_{\eta})$. Under bounded update sensitivity  (enforced via gradient clipping), SP-DP satisfies -differential privacy. By confining the majority of the noise to the null space (which contains high-frequency sensor artifacts), SP-DP preserves the critical low-rank eigenspaces required for accurate localization.




==> paper_content/05_future_work.tex <==
\section{Future Work and Limitations}
\label{sec:fw_limit}

\subsection{Future Work}
\label{sec:future_work}



\subsection{Limitations}
\label{sec:limitations}


==> paper_content/06_conclusions.tex <==
\section{Conclusions}
\label{sec:conclusion}

